Recurrent Spatial Transformer Networks

We integrate the recently proposed spatial transformer network (SPN) [Jaderberg et. al 2015] into a recurrent neural network (RNN) to form an RNN-SPN model. We use the RNN-SPN to classify digits in cluttered MNIST sequences. The proposed model achieves a single digit error of 1.5% compared to 2.9% for a convolutional networks and 2.0% for convolutional networks with SPN layers. The SPN outputs a zoomed, rotated and skewed version of the input image. We investigate different down-sampling factors (ratio of pixel in input and output) for the SPN and show that the RNN-SPN model is able to down-sample the input images without deteriorating performance. The down-sampling in RNN-SPN can be thought of as adaptive down-sampling that minimizes the information loss in the regions of interest. We attribute the superior performance of the RNN-SPN to the fact that it can attend to a sequence of regions of interest.

==> contributions.tex <==
%!TEX root = report.tex
\section{AUTHORS CONTRIBUTIONS}


==> discussion.tex <==
%!TEX root = report.tex
\section{Discussion and Conclusion} % (fold)


==> method.tex <==
%!TEX root = report.tex
\section{Materials and Methods}%

